Three-Body Scattering for Generative Modeling

Modern generative models typically rely on an adversarial critic, a prescribed noise-to-data path, or an autoregressive factorization. Instead, we show that a proper distributional energy can induce sample-level motion and provide direct regression supervision for a one-step generator. Three-Body Scattering Modeling (TBSM) for generation turns the energy distance into a constant-size per-projectile interaction: each projectile is attracted toward one real source and repelled from one independently generated source. Conditioned on the projectile and its condition, its expectation equals the $2$-Wasserstein gradient-flow velocity of $\frac12D_E^2(P_{\theta},Q)$. A batch of $B$ frozen-target events yields $O(B)$ sample-level losses, each using one reference for its condition instead of the minibatch-wide all-pairs field used by methods such as Drifting Models. Tracking this conditional expectation online can reduce field noise. Using scattering in frozen image features, TBSM trains one-step generators on ImageNet-256, achieving FID${}=2.23$ with pixel-space PixelDiT-XL and FID${}=1.63$ with latent-space DiT-XL at NFE${}=1$. We provide a design map relating diffusion-related supervision, Drift-like dynamics, and GAN-like objectives. These results establish tracked scattering as a route to high-dimensional one-step generation. Code: https://github.com/sp12138/TBSM.

==> resources/figures/lambda_rho_plane.tex <==
\begin{tikzpicture}[
        remember picture,
        x=1cm,
        y=1cm,
        point/.style={
                circle,
                fill=darkred,
                draw=white,
                line width=0.7pt,
                minimum size=6.2pt,
                inner sep=0pt
            },
        labelbox/.style={
                align=center,
                font=\scriptsize,
                fill=white,
                fill opacity=0.92,
                text opacity=1,
                rounded corners=2pt,
                inner xsep=2pt,
                inner ysep=2.5pt,
                text width=2.15cm,
                text=black!82
            },
        smallmath/.style={font=\scriptsize, text=black!62},
        axislabel/.style={font=\footnotesize, text=black!72},
        family/.style={align=center, font=\footnotesize\bfseries, text=darkblue}
    ]
    \def\W{5.20}
    \def\H{5.20}

    \path[fill=white] (-0.84,-0.88) rectangle (\W+0.30,\H+0.30);
    \path[fill=darkgreen!6] (0,0) rectangle (0.5*\W,0.5*\H);
    \path[fill=darkred!8] (0.5*\W,0) rectangle (\W,0.5*\H);
    \path[fill=darkblue!7] (0,0.5*\H) rectangle (0.5*\W,\H);
    \path[fill=purple!8] (0.5*\W,0.5*\H) rectangle (\W,\H);
    \draw[step=0.52, draw=black!7, line width=0.35pt] (0,0) grid (\W,\H);
    \draw[draw=black!18, line width=0.5pt] (0.5*\W,0) -- (0.5*\W,\H);
    \draw[draw=black!18, line width=0.5pt] (0,0.5*\H) -- (\W,0.5*\H);
    \draw[draw=black!45, line width=0.65pt, rounded corners=3pt] (0,0) rectangle (\W,\H);

    \node[
    family,
    fill=white,
    fill opacity=0.92,
    text opacity=1,
    draw=darkblue!18,
    rounded corners=3pt,
    inner xsep=6pt,
    inner ysep=4pt
    ] at (0.5*\W,0.5*\H)
    {\method{} family\\{\normalfont\scriptsize $\lambda$-weighted / tracked targets}};

    \coordinate (tbsmPlaneDiff) at (0,0);
    \coordinate (tbsmPlaneGan) at (\W,0);
    \coordinate (tbsmPlaneDrift) at (0,\H);
    \coordinate (tbsmPlaneMain) at (\W,\H);

    \node[point] at (tbsmPlaneDiff) {};
    \node[point] at (tbsmPlaneGan) {};
    \node[point] at (tbsmPlaneDrift) {};
    \node[point] at (tbsmPlaneMain) {};

    \node[labelbox, anchor=north west]
    at ([xshift=5pt,yshift=-5pt]tbsmPlaneDrift)
    {\textbf{Instant scattering}\\[-1pt]
        \textcolor{black!62}{$\rho=0,\lambda=1$}\\[-1pt]
        (\textbf{Drift-like}; \citealp{deng2026drifting})};
    \node[labelbox, anchor=north east]
    at ([xshift=-5pt,yshift=-5pt]tbsmPlaneMain)
    {\textbf{Tracked scattering}\\[-1pt]
        \textcolor{black!62}{$\rho=1,\lambda=1$}\\[-1pt]
        (\textbf{energy-distance endpoint}; \textbf{ours})};
    \node[labelbox, anchor=south west]
    at ([xshift=5pt,yshift=5pt]tbsmPlaneDiff)
    {\textbf{Inter-only scattering}\\[-1pt]
        \textcolor{black!62}{$\rho=0,\lambda=0$}\\[-1pt]
        (\textbf{diffusion-related}; \citealp{ho2020denoising})};
    \node[labelbox, anchor=south east]
    at ([xshift=-5pt,yshift=5pt]tbsmPlaneGan)
    {\textbf{Fake-to-real}\\[-1pt]
        \textbf{interpolation}\\[-1pt]
        \textcolor{black!62}{$\rho=1,\lambda=0$}\\[-1pt]
        (\textbf{GAN-like}; \citealp{goodfellow2014generative})};

    \draw[->, line width=0.75pt, draw=black!62]
    (0,-0.34) -- (\W,-0.34)
    node[midway, below=3pt, axislabel]
    {tracked-supervision weight $\rho$};
    \draw[->, line width=0.75pt, draw=black!62]
    (-0.34,0) -- (-0.34,\H)
    node[midway, above=3pt, rotate=90, axislabel]
    {intra-source weight $\lambda$};

    \node[smallmath, anchor=north] at (0,-0.42) {$0$};
    \node[smallmath, anchor=north] at (\W,-0.42) {$1$};
    \node[smallmath, anchor=east] at (-0.42,0) {$0$};
    \node[smallmath, anchor=east] at (-0.42,\H) {$1$};
\end{tikzpicture}%

